Frontier LLMs are effective batch optimizers: Assessing reasoning models in continuous and discrete settings

Frontier large language models (LLMs) have become attractive priors for optimization due to their large-scale pretraining that enables them to navigate a variety of optimization settings. However, the effectiveness of modern reasoning LLMs in batch optimization settings remains underexplored. Here we investigate the performance of the current generation of frontier LLMs as batch optimizers in both continuous and discrete settings. We find that while LLMs are competitive zero-shot batch optimizers for numerical test functions, their performance is brittle compared to classical non-LLM optimization approaches. However, LLM priors are significantly better in semantically rich settings, indicating that their batch optimization behavior is highly effective when navigating and reasoning over the discrete spaces most similar in structure to their pretraining data.

==> shortened_sections/abstract.tex <==
Frontier large language models (LLMs) have become attractive priors for optimization due to their large-scale pretraining that enables them to navigate a variety of optimization settings. However, the effectiveness of modern reasoning LLMs in batch optimization settings remains underexplored.
%and is an open area of research with implications in a variety of fields ranging from numerical optimization to molecular design.
Here we investigate the performance of the current generation of frontier LLMs as batch optimizers in both continuous and discrete settings. We find that while LLMs are competitive zero-shot batch optimizers for numerical test functions, their performance is brittle compared to classical non-LLM optimization approaches. However, LLM priors are significantly better in semantically rich settings, indicating that their batch optimization behavior is highly effective when navigating and reasoning over the discrete spaces most similar in structure to their pretraining data. 


==> shortened_sections/body.tex <==
\section{Introduction}
\label{sec:introduction}
Frontier large language models (LLMs) have become increasingly powerful with each new generation due to the continued development of pretraining corpora and reinforcement learning protocols, instilling these models with exceptional reasoning capabilities that enable them to tackle lengthier and more complex tasks. This has made them attractive for a variety of applications, most notably in programming~\citep{research_composer_2026}, mathematics~\citep{shao_deepseekmath_2024}, and more recently, scientific discovery~\citep{chennakesavalu_evaluating_2026,narayanan_training_2025}. While this continued evolution in LLM capabilities is remarkable, it remains unclear how effective these models have become for black-box optimization (BBO)~\citep{alarie_two_2021,audet_derivative-free_2026} settings where the evaluation of a target objective function is expensive, rendering brute force optimization intractable. This is a ubiquitous scenario in scientific settings like small-molecule drug discovery where candidate evaluations for a proposed small-molecule design require a high investment of time and resources, meaning that the evaluation budget is highly restricted against a combinatorially complex design space~\citep{ertl_cheminformatics_2003,ertl_estimation_2009}. 

In this work we investigate the performance of the Anthropic family of models (Sonnet 4.6~\citep{anthropic_introducing_2026}, Opus 4.8~\citep{_introducing_op48}, and Opus 5~\citep{_introducing_a}) as batch optimizers for a collection of continuous and discrete BBO tasks. For evaluation over a continuous search space, we use a set of well-known optimization functions of varying dimensionality, taking care to disguise their domains and ranges to minimize memorization exploitation from the model. For the discrete setting, we choose molecular optimization against the set of oracles detailed in the practical molecular optimization (PMO)~\citep{gaoSampleEfficiencyMatters2022} benchmark. Overall, we find that frontier reasoning LLMs can be effective but brittle numerical optimizers, with performance that rivals classical Bayesian Optimization with a Gaussian process surrogate and an expected improvement acquisition function, but the general performance depends heavily on task transformations, dimensionality, and batch size. However, we show that in the discrete molecular optimization setting, the frontier reasoning LLMs are both highly performant and sample efficient, frequently beating specialist methods with only a fraction of the oracle sampling budget. 

\section{Related work}
\label{sec:related-work}

{\noindent
\textbf{Bayesian Optimization}
Bayesian Optimization (BO) is a global optimization method for black-box optimization \citep{frazierTutorialBayesianOptimization2018}. It is an active learning method that employs a probabilistic surrogate model, 
$\hat f$, over the input domain $\mathcal H$ to characterize the posterior predictive distribution of the objective, together with an acquisition function, $\alpha(h; \hat f, \mathcal D)$, that quantifies the utility of evaluating an input $h \in \mathcal H$ conditioned on a fitted surrogate model $\hat f$ and measured dataset $\mathcal D$ to guide the selection of the next point. Gaussian processes (GPs) \citep{Rasmussen2006Gaussian} are a typical choice of surrogate model given the intuitive prior defined via the kernel and analytically tractable posterior inference \citep{snoekPracticalBayesianOptimization2012}. Common acquisition functions include both upper confidence bound (UCB) and expected improvement (EI), which balance exploration of the landscape and exploitation of promising regions. BO is a popular choice to optimize black-box functions across many domains, such as materials science~\citep{chitturi_targeted_2024}, chemistry~\citep{nambiar_bayesian_2022}, biology~\citep{li_biobo_2025}, and robotics~\citep{martinez-cantin_funneled_2019}.

% {\noindent
% \textbf{Pretrained models for optimization}
% Prior work has explored the application of pretrained models to optimization tasks. Broadly, these works can be classified into two regimes: (1) pretraining transformer models to mimic tokenized optimization trajectories on synthetic tasks \citep{song_reinforced_2024,meindlZeroShotOptZeroShotPretrained2025} and (2) leveraging pretrained LLMs to enhance individual components of the BO loop~\citep{liuLargeLanguageModels2024,ramosBayesianOptimizationCatalysis2025}. Most similar to our work are \citet{yangLargeLanguageModels2024} and \citet{huangExploringTruePotential2024}, both of which utilize a prompt-based approach as a stand-in for a full optimization policy. But these methods do not explore batched LLM optimization policies applied to standard BO test functions nor do they apply these approaches to molecular optimization. Most importantly, LLM capabilities have substantially improved since these prior studies were conducted. Hence, it is important to revisit these methodologies using significantly more capable frontier models.
% }

{\noindent
\textbf{Molecular optimization}
Optimizing molecular properties is a key challenge in the development of novel functional materials, such as pharmaceuticals, photovoltaics, and batteries. Broadly, there are two strategies to improve desired properties: (1) forward search in a predefined library, where molecules are \emph{screened} according to the property itself (or some surrogate thereof) and (2) inverse design, where molecules are \emph{generated} based on a specification of the desired properties \citep{sanchez-lengelingInverseMolecularDesign2018}. LLMs have been used in a variety of ways for molecular optimization: as generators of property-optimized molecules \citep{navratilGPMoLFormerSimTestTime2025,bagalMolGPTMolecularGeneration2021,kopfSampleEfficientGenerative2026,rankovicLargeLanguageModels2026}, molecular representation learners for use in property prediction \citep{freyNeuralScalingDeep2023,ahmadChemBERTa2ChemicalFoundation2022}, property predictors themselves, and augmentations to individual components of closed-loop optimization protocols \citep{ramosBayesianOptimizationCatalysis2025,ranExLLMExperienceEnhancedLLM2025,wangEfficientEvolutionarySearch2025}}.

\section{Experimental design}
We first examine the performance of the frontier LLMs on a set of synthetic optimization tasks using classical test functions with known optima: Branin, Hartmann-3, Hartmann-6, Ackley, and Rastrigin. For a summary of these synthetic test functions and their optima, refer to Appendix~\ref{app:synthetic-functions}. For each of these functions, we normalize the domain to $[0,1]^d$ and perform any necessary negations such that every task can be framed as a maximization. We then evaluate each LLM in both single- and multi-turn settings with batch sizes $q=1,2,4$ where the model emits a collection of points $\{h_i\}_{i=1}^q\subset[0,1]^d$ at each trajectory step. To ensure that the overall optimization budget is matched, we fix a total run budget of $N=120$ with $2d$ initial points based on the dimensionality of the problem, and where the length of each trajectory for each batch size is computed as $N/q$. In addition to testing on the original version of these functions, we also test on a disguised variation of these test functions by applying a bijection on the domain $\mathcal{T}:[0,1]^d \rightarrow [0,1]^d$ and an affine transformation on the outputs (see Appendix~\ref{app:synthetic-functions} for more details). We compare the LLM-based optimization policies to both a BO policy with a GP surrogate and EI acquisition function (``GP-EI'') as well as a random baseline.

For a semantically richer optimization task, we assess the LLMs on the suite of molecular optimization tasks described in PMO~\citep{gaoSampleEfficiencyMatters2022} which tests the ability of different methods for maximizing small-molecule oracles in a sample-efficient manner. Unlike the synthetic test functions, these optimization problems naturally admit a discrete, natural-language representation via SMILES~\citep{weininger_smiles_1988} strings, and there is no analytic optimum for these oracles. We choose this molecular optimization task as opposed to other natural-language benchmarks because of the availability of cheap and deterministic oracle functions, meaning there is no ambiguity with regard to assessing improvement on specific tasks. We evaluate all three frontier LLMs on all 23 PMO oracles across five seeds, again testing both single-turn and multi-turn settings. We compare the performance of the frontier LLMs against all of the other methods included in the original PMO paper and some additional ones. Unlike the 10000 oracle call budget that was used in the original study, we restrict our LLM evaluations to a very low-budget setting consisting of 10 initial molecules followed by 20 batches of 10 for a total oracle budget of 210. For comparing across all the methods, we use Top-10 AUC and the Top-10 mean, where the former is useful for gauging sample efficiency. Where applicable, we use early stopping in a manner consistent with the method's original publication.

\section{Results}

\subsection{Optimization on synthetic test functions}\label{sec:synth_tasks}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/Figure1.pdf}
    \caption{A comparison of the simple regret of Opus 5 multi-turn against GP-EI for batch sizes $q=1,2,4$ across all five synthetic tasks and both disguised and plain variants. Stars indicate cases where the policy achieved a regret that is truly zero up to machine precision. Bars are $\pm$1 standard error (SE) computed across five seeds.}
    \label{fig:opus_synthetic_comparison}
\end{figure}

Figure~\ref{fig:opus_synthetic_comparison} compares Opus 5 multi-turn against GP-EI on the full panel of synthetic test functions for both the plain and disguised variations and batch sizes $q=1,2,4$. We choose Opus 5 multi-turn because it is the strongest-performing LLM condition when compared to its own single-turn variation and the performance of Opus 4.8 and Sonnet 4.6 (see Appendix~\ref{app:synth_optim}). We see that across all batch sizes, Opus 5 multi-turn outperforms GP-EI on a majority of the 10 optimization tasks, with the LLM regret slightly degrading with increasing batch size as evidenced by the upward vertical drift observed for the tasks other than the plain Ackley function and the two Branin variations. In contrast, the performance of GP-EI remains consistent across batch sizes for both the disguised and plain variations of the tasks, indicating that batch size does not have a significant positive effect on the final attained regret for the non-LLM method. Comparing across the disguised and plain variations of the tasks, we see that for Opus 5, the model consistently performs worse on the disguised variation compared to the plain variation of each task whereas GP-EI again maintains a consistent level of performance. The discrepancy for the LLM is most noticeable in the cases of the Ackley and Rastrigin tasks, where the model attains an average simple regret of exactly zero for the $q=1$ and $q=4$ plain cases but not for the disguised variants. To understand this discrepancy, we examine the optimization trajectory of the Opus 5 $q=1$ scan across all 10 variations grouped by task as shown in Figure~\ref{fig:plain_disguised_task_comp}. We see that for the lower-dimensional Branin and Hartmann-3 tasks, the average simple regret eventually reaches the low regret floor over the course of the optimization for both the disguised and plain tasks, with the LLM performing comparably well on the disguised task compared to the plain variations. However, for the higher-dimensional tasks Hartmann-6, Ackley, and Rastrigin, disguising both the domain and the range leads to a significant loss in performance, with the model no longer able to attain the zero regret optimum. In addition to the discrepancies between the disguised and plain variants of the tasks and the decreased optimization performance as a function of problem dimensionality, we find that models sometimes recognize the topology of the function they are navigating by reasoning over the evaluated points and then use that knowledge to refine their optimization (see Appendix~\ref{app:synth_mem_analysis} for a more detailed memorization analysis). 

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/Figure2.pdf}
    \caption{Simple regret versus number of function evaluations for Opus 5 in the multi-turn setting with $q=1$ for all five tasks, with both variations shown. Solid lines represent the mean across five seeds and shaded bands represent $\pm$1 SE. A dotted line corresponds to 0 regret (up to machine precision).}
    \label{fig:plain_disguised_task_comp}
\end{figure}

\subsection{Molecular optimization on PMO}
We now turn to evaluating these reasoning LLMs on their performance in discrete optimization, a more natural setting given that autoregressive LLMs are trained to navigate discrete spaces such as natural language. We use the PMO molecular optimization benchmark which focuses on maximization under a series of deterministic black-box small-molecule oracles with comparisons across a number of different methods. We restrict our LLM budget to only 210 oracle evaluations, corresponding to an initial set of 10 molecules randomly sampled from the ZINC 250K dataset \citep{tingle_zinc22xe5f8a_2023} followed by 20 batches of 10. Comparing across LLM generations, we find that model performance increases with newer generations and multi-turn performance exceeds the corresponding single-turn performance, resulting in Opus 5 multi-turn once again being the best-performing condition. Indeed, on the full set of 23 oracles, Opus 5 is the best by Top-10 AUC in 17 out of the 23 cases, and the best by Top-10 mean in 20 out of the 23 cases (see Appendix~\ref{app:inter_llm_on_pmo}). 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{figures/Figure3.pdf}
%     \caption{A comparison of Sonnet 4.6, Opus 4.8, and Opus 5 on a selected set of isomer, rediscovery, similarity, and MPO tasks, with all three models evaluated in both single- and multi-turn settings. The top row shows the Top-10 AUC score and the bottom row shows the Top-10 mean score, with error bars corresponding to $\pm$1 SE over five seeds.}
%     \label{fig:inter_llm_comp_pmo}
% \end{figure}

Continuing with Opus 5 multi-turn, we next compare its performance against a subset of nine specialist methods on the same tasks. This includes a mix of methods tested in the original PMO paper and methods that we have reproduced, such as SMILES Augmented Memory~\citep{guoAugmentedMemorySampleEfficient2024}, GenMol~\citep{lee_genmol_2025}, ExLLM~\citep{ranExLLMExperienceEnhancedLLM2025}, and MolLEO~\citep{wangEfficientEvolutionarySearch2025}. Some additional methods such as LICO~\citep{nguyenLICOLargeLanguage2025} and GP-MoLFormer-SIM~\citep{navratilGPMoLFormerSimTestTime2025} also benchmark on the PMO task set, but these methods do not provide any code or optimization trajectories necessary for our analysis; as such, we compare our best results against their methods in Appendix~\ref{app:non-repro-comparison}. Figure~\ref{fig:llm_v_specialist_pmo} shows the Top-10 mean as a function of the oracle call number for a subset of the tasks, ranging from 1 to the maximum budget of 210. We see that in the low-budget regime, the reasoning LLM is a competitive optimizer, exceeding the Top-10 mean of some bespoke deep-learning-based methods like REINVENT~\citep{blaschke_reinvent_2020} and SynNet~\citep{gao_amortized_2022} as well as BO-based methods and search methods. When compared to more specialized methods like GenMol, MolLEO, and ExLLM, Opus 5 maintains comparable performance for oracles such as thiothixene rediscovery and osimertinib MPO, but falls behind specialist methods on the selected isomer and mestranol similarity tasks.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/smaller_versions/Figure4.pdf}
    \caption{Top-10 mean reward curves for the selected isomer, rediscovery, similarity, and MPO tasks, comparing Opus 5 multi-turn against nine selected specialist methods for each oracle across a budget of 210 oracle evaluations. The shaded regions correspond to $\pm$1 SE over the five seeds.}
    \label{fig:llm_v_specialist_pmo}
\end{figure}

While the differences in performance between Opus 5 and these alternative methods can appear especially large, it is worth noting that these approaches use either a carefully trained specialist architecture already tuned on drug-like molecules (as in the case of GenMol) or an LLM to drive the optimization with significantly more scaffolding around the problem (as in the case of MolLEO and ExLLM). GenMol, especially, has an advantage in these tasks because it was trained on an extensive dataset of small molecules from the SAFE dataset~\citep{noutahi_gotta_2023}, meaning it is specialized for generating drug-like compounds. This is a possible source of superior performance when compared to the LLM-based methods where it wins 13 of 23 oracles by Top-10 AUC under an oracle call budget of 210. However, we note that in terms of Top-10 mean at a budget of 210, GenMol is comparable to Opus 5 multi-turn (0.590 average across oracles for GenMol versus 0.596 for Opus 5) with ExLLM being the best-performing method with an average of 0.738 across oracles (see Appendix~\ref{app:molec_optim}). In contrast to these methods, Opus 5 is used directly without any additional tuning or scaffolding, so the fact that the frontier reasoning LLM maintains comparable performance is especially impressive and indicative of the evolving capabilities of these models. Additionally, comparing the LLM performance in the discrete setting to the performance in the continuous setting in Section~\ref{sec:synth_tasks}, it is clear that the reasoning LLM functions as a better batch optimizer in discrete settings.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/smaller_versions/Figure5.pdf}
    \caption{Comparison of the number of additional oracle calls required for specialist methods' Top-10 mean to reach LLM performance across the selected isomer, rediscovery, similarity, and MPO tasks. The fold value is computed using the median of the first step to reach LLM performance, taken over the set of seeds that reached LLM-level performance. Methods that never reach LLM performance within their optimization are represented as hatched bars.}
    \label{fig:llm_v_specialist_fold}
\end{figure}

We can extend our analysis by measuring the performance improvement when the full oracle budget is allowed. Doing this allows us to quantify how many additional (or fewer) oracle calls are required before a given method achieves performance comparable to that of the LLM, resulting in a budget multiplier where a lower multiplier indicates a more sample-efficient method. Figure~\ref{fig:llm_v_specialist_fold} shows the comparison for the same selection of tasks and methods. We observe that GenMol, ExLLM, and MolLEO are more sample efficient than Opus 5, all of them taking fewer than 210 oracle calls to match the performance in the isomer task. ExLLM is especially consistent, achieving a multiplier of $\leq1\times$ across the four selected tasks, with GenMol as a close second where it was only less efficient than Opus 5 on the thiothixene rediscovery task. For the other selected methods, we see that even the most sample-efficient of this group requires at least three times as many oracle calls to achieve comparable performance, with many methods requiring 20--40 times as many oracle calls. Certain methods also never reach LLM performance throughout the course of their optimization, as shown by the performance of screening in three of the four tasks, SMILES GA in thiothixene rediscovery, and SynNet in osimertinib MPO. Having compared across both the raw performance and sample efficiency axes, we see that while frontier reasoning LLMs still underperform carefully trained and highly scaffolded specialist approaches, their zero-shot performance is still competitive with a range of optimization methods while maintaining sample efficiency. This highlights their utility as batch optimizers in discrete settings, with future iterations of frontier models likely leading to continued improvements in this regard. For full results on the PMO tasks, see Appendix~\ref{app:molec_optim}. 

\section{Conclusion}

Here we present an analysis of frontier reasoning LLMs as batch optimizers for both continuous and discrete BBO tasks. We show that while LLMs are competitive with GP-EI on synthetic test functions, their performance is brittle and dependent on factors such as batch size, task dimensionality, and extent of transformation applied. However, in the discrete setting of molecular optimization, LLMs are both highly performant and sample-efficient optimizers, beating a host of bespoke methods without additional tuning or problem scaffolding and underperforming only when compared to specially trained or highly structured strategies. In the context of BBO-type problems, our results show that frontier reasoning LLMs are powerful priors for batch discrete optimization without any additional tuning, with potentially wide-reaching utility. Immediate future directions for our work include extending our analysis to new numerical and discrete settings to evaluate LLM performance on additional BBO problem formulations and designing mid- and post-training protocols for enhancing open-weight reasoning LLM performance on BBO tasks.


==> shortened_tables/frontier_pmo_table.tex <==
% Requires: \usepackage{booktabs}   % (amsmath for \boldmath already standard)
\begin{table*}[htbp]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Top-10 AUC at a 210-call budget on all 23 PMO oracles.} The three frontier LLMs, each in single- and multi-turn mode, scored as the area under the running Top-10 mean curve out to 210 oracle calls. Mean $\pm$1 SE over five seeds; higher is better; \textbf{bold} = best arm for that oracle. The final row counts, for each arm, how many of the 23 oracles it wins (co-winners on an exact tie each count).}
\label{tab:frontier-pmo-auc}
\begin{tabular}{@{}l *{6}{c}@{}}
\toprule
Oracle & \multicolumn{2}{c}{Sonnet 4.6} & \multicolumn{2}{c}{Opus 4.8} & \multicolumn{2}{c}{Opus 5} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & single-turn & multi-turn & single-turn & multi-turn & single-turn & multi-turn \\
\midrule
albuterol\_similarity & $ 0.136 \pm 0.025 $ & $ 0.460 \pm 0.022 $ & $ 0.449 \pm 0.026 $ & $ 0.355 \pm 0.060 $ & $ 0.560 \pm 0.054 $ & {\boldmath$ 0.739 \pm 0.020 $} \\
amlodipine\_mpo & $ 0.308 \pm 0.038 $ & $ 0.447 \pm 0.005 $ & $ 0.457 \pm 0.008 $ & $ 0.471 \pm 0.010 $ & $ 0.473 \pm 0.009 $ & {\boldmath$ 0.485 \pm 0.010 $} \\
celecoxib\_rediscovery & $ 0.106 \pm 0.010 $ & $ 0.386 \pm 0.009 $ & $ 0.395 \pm 0.021 $ & $ 0.401 \pm 0.033 $ & $ 0.487 \pm 0.036 $ & {\boldmath$ 0.594 \pm 0.076 $} \\
deco\_hop & $ 0.424 \pm 0.050 $ & $ 0.560 \pm 0.006 $ & $ 0.551 \pm 0.005 $ & $ 0.540 \pm 0.012 $ & $ 0.556 \pm 0.006 $ & {\boldmath$ 0.583 \pm 0.026 $} \\
drd2 & $ 0.227 \pm 0.103 $ & $ 0.337 \pm 0.121 $ & $ 0.320 \pm 0.094 $ & $ 0.393 \pm 0.116 $ & $ 0.288 \pm 0.119 $ & {\boldmath$ 0.524 \pm 0.091 $} \\
fexofenadine\_mpo & $ 0.343 \pm 0.093 $ & $ 0.633 \pm 0.013 $ & $ 0.642 \pm 0.013 $ & $ 0.624 \pm 0.017 $ & $ 0.654 \pm 0.018 $ & {\boldmath$ 0.680 \pm 0.014 $} \\
gsk3b & $ 0.088 \pm 0.052 $ & $ 0.296 \pm 0.044 $ & $ 0.266 \pm 0.037 $ & $ 0.275 \pm 0.051 $ & $ 0.356 \pm 0.077 $ & {\boldmath$ 0.609 \pm 0.078 $} \\
isomers\_c7h8n2o2 & $ 0.005 \pm 0.003 $ & $ 0.158 \pm 0.078 $ & $ 0.052 \pm 0.032 $ & {\boldmath$ 0.210 \pm 0.058 $} & $ 0.101 \pm 0.036 $ & $ 0.158 \pm 0.045 $ \\
isomers\_c9h10n2o2pf2cl & $ 0.005 \pm 0.002 $ & {\boldmath$ 0.122 \pm 0.044 $} & $ 0.043 \pm 0.025 $ & $ 0.085 \pm 0.036 $ & $ 0.089 \pm 0.037 $ & $ 0.097 \pm 0.037 $ \\
jnk3 & $ 0.066 \pm 0.042 $ & $ 0.181 \pm 0.042 $ & $ 0.253 \pm 0.042 $ & $ 0.179 \pm 0.040 $ & $ 0.212 \pm 0.042 $ & {\boldmath$ 0.308 \pm 0.060 $} \\
median1 & $ 0.059 \pm 0.018 $ & $ 0.152 \pm 0.008 $ & $ 0.141 \pm 0.012 $ & $ 0.150 \pm 0.011 $ & $ 0.165 \pm 0.012 $ & {\boldmath$ 0.183 \pm 0.013 $} \\
median2 & $ 0.064 \pm 0.024 $ & $ 0.182 \pm 0.008 $ & $ 0.190 \pm 0.012 $ & $ 0.185 \pm 0.011 $ & {\boldmath$ 0.195 \pm 0.011 $} & $ 0.195 \pm 0.013 $ \\
mestranol\_similarity & $ 0.126 \pm 0.038 $ & $ 0.271 \pm 0.061 $ & $ 0.318 \pm 0.024 $ & $ 0.313 \pm 0.023 $ & $ 0.314 \pm 0.018 $ & {\boldmath$ 0.345 \pm 0.022 $} \\
osimertinib\_mpo & $ 0.395 \pm 0.112 $ & $ 0.704 \pm 0.016 $ & $ 0.708 \pm 0.015 $ & $ 0.676 \pm 0.028 $ & $ 0.705 \pm 0.019 $ & {\boldmath$ 0.722 \pm 0.014 $} \\
perindopril\_mpo & $ 0.180 \pm 0.068 $ & $ 0.431 \pm 0.010 $ & $ 0.392 \pm 0.041 $ & $ 0.367 \pm 0.056 $ & $ 0.427 \pm 0.006 $ & {\boldmath$ 0.436 \pm 0.006 $} \\
qed & $ 0.288 \pm 0.060 $ & $ 0.860 \pm 0.011 $ & $ 0.637 \pm 0.127 $ & $ 0.625 \pm 0.067 $ & {\boldmath$ 0.886 \pm 0.006 $} & $ 0.712 \pm 0.019 $ \\
ranolazine\_mpo & $ 0.241 \pm 0.093 $ & $ 0.538 \pm 0.037 $ & $ 0.495 \pm 0.046 $ & $ 0.506 \pm 0.035 $ & $ 0.590 \pm 0.024 $ & {\boldmath$ 0.606 \pm 0.011 $} \\
scaffold\_hop & $ 0.378 \pm 0.052 $ & $ 0.356 \pm 0.068 $ & $ 0.433 \pm 0.009 $ & $ 0.433 \pm 0.010 $ & $ 0.393 \pm 0.041 $ & {\boldmath$ 0.456 \pm 0.009 $} \\
sitagliptin\_mpo & $ 0.012 \pm 0.003 $ & $ 0.062 \pm 0.024 $ & $ 0.048 \pm 0.024 $ & $ 0.072 \pm 0.019 $ & {\boldmath$ 0.098 \pm 0.030 $} & $ 0.053 \pm 0.012 $ \\
thiothixene\_rediscovery & $ 0.113 \pm 0.035 $ & $ 0.280 \pm 0.014 $ & $ 0.257 \pm 0.027 $ & $ 0.262 \pm 0.009 $ & $ 0.294 \pm 0.005 $ & {\boldmath$ 0.377 \pm 0.011 $} \\
troglitazone\_rediscovery & $ 0.082 \pm 0.009 $ & $ 0.266 \pm 0.005 $ & $ 0.216 \pm 0.023 $ & $ 0.232 \pm 0.015 $ & $ 0.266 \pm 0.008 $ & {\boldmath$ 0.394 \pm 0.097 $} \\
valsartan\_smarts & $ 0.000 \pm 0.000 $ & $ 0.000 \pm 0.000 $ & $ 0.000 \pm 0.000 $ & $ 0.000 \pm 0.000 $ & $ 0.000 \pm 0.000 $ & {\boldmath$ 0.363 \pm 0.052 $} \\
zaleplon\_mpo & $ 0.042 \pm 0.012 $ & $ 0.086 \pm 0.012 $ & $ 0.084 \pm 0.027 $ & {\boldmath$ 0.136 \pm 0.014 $} & $ 0.106 \pm 0.032 $ & $ 0.084 \pm 0.022 $ \\
\midrule
Mean (23 oracles) & $ 0.160 $ & $ 0.338 $ & $ 0.319 $ & $ 0.326 $ & $ 0.357 $ & $ 0.422 $ \\
Oracles won (best of 23) & 0 & 1 & 0 & 2 & 3 & 17 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[htbp]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Top-10 mean at a 210-call budget on all 23 PMO oracles.} The mean oracle score of the 10 best molecules found within 210 oracle calls, for the three frontier LLMs in single- and multi-turn mode. Mean $\pm$1 SE over five seeds; higher is better; \textbf{bold} = best arm for that oracle. The final row counts, for each arm, how many of the 23 oracles it wins (co-winners on an exact tie each count).}
\label{tab:frontier-pmo-mean}
\begin{tabular}{@{}l *{6}{c}@{}}
\toprule
Oracle & \multicolumn{2}{c}{Sonnet 4.6} & \multicolumn{2}{c}{Opus 4.8} & \multicolumn{2}{c}{Opus 5} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & single-turn & multi-turn & single-turn & multi-turn & single-turn & multi-turn \\
\midrule
albuterol\_similarity & $ 0.448 \pm 0.021 $ & $ 0.659 \pm 0.037 $ & $ 0.549 \pm 0.042 $ & $ 0.511 \pm 0.033 $ & $ 0.775 \pm 0.082 $ & {\boldmath$ 1.000 \pm 0.000 $} \\
amlodipine\_mpo & $ 0.515 \pm 0.011 $ & $ 0.524 \pm 0.011 $ & $ 0.515 \pm 0.011 $ & $ 0.554 \pm 0.010 $ & $ 0.547 \pm 0.009 $ & {\boldmath$ 0.564 \pm 0.011 $} \\
celecoxib\_rediscovery & $ 0.363 \pm 0.014 $ & $ 0.537 \pm 0.041 $ & $ 0.476 \pm 0.027 $ & $ 0.578 \pm 0.069 $ & $ 0.767 \pm 0.087 $ & {\boldmath$ 1.000 \pm 0.000 $} \\
deco\_hop & $ 0.585 \pm 0.005 $ & $ 0.605 \pm 0.004 $ & $ 0.587 \pm 0.006 $ & $ 0.602 \pm 0.009 $ & $ 0.597 \pm 0.007 $ & {\boldmath$ 0.661 \pm 0.056 $} \\
drd2 & $ 0.477 \pm 0.159 $ & $ 0.514 \pm 0.133 $ & $ 0.568 \pm 0.137 $ & $ 0.683 \pm 0.171 $ & $ 0.395 \pm 0.137 $ & {\boldmath$ 0.945 \pm 0.028 $} \\
fexofenadine\_mpo & $ 0.674 \pm 0.024 $ & $ 0.714 \pm 0.016 $ & $ 0.700 \pm 0.016 $ & $ 0.732 \pm 0.015 $ & $ 0.733 \pm 0.021 $ & {\boldmath$ 0.770 \pm 0.015 $} \\
gsk3b & $ 0.287 \pm 0.064 $ & $ 0.413 \pm 0.060 $ & $ 0.355 \pm 0.048 $ & $ 0.452 \pm 0.042 $ & $ 0.474 \pm 0.095 $ & {\boldmath$ 0.775 \pm 0.068 $} \\
isomers\_c7h8n2o2 & $ 0.036 \pm 0.024 $ & $ 0.375 \pm 0.149 $ & $ 0.119 \pm 0.060 $ & $ 0.487 \pm 0.135 $ & $ 0.404 \pm 0.147 $ & {\boldmath$ 0.522 \pm 0.120 $} \\
isomers\_c9h10n2o2pf2cl & $ 0.026 \pm 0.014 $ & $ 0.300 \pm 0.104 $ & $ 0.064 \pm 0.037 $ & $ 0.171 \pm 0.064 $ & $ 0.184 \pm 0.075 $ & {\boldmath$ 0.328 \pm 0.110 $} \\
jnk3 & $ 0.151 \pm 0.037 $ & $ 0.247 \pm 0.048 $ & $ 0.366 \pm 0.087 $ & $ 0.245 \pm 0.057 $ & $ 0.290 \pm 0.052 $ & {\boldmath$ 0.495 \pm 0.098 $} \\
median1 & $ 0.158 \pm 0.009 $ & $ 0.193 \pm 0.010 $ & $ 0.162 \pm 0.015 $ & $ 0.196 \pm 0.016 $ & $ 0.212 \pm 0.022 $ & {\boldmath$ 0.260 \pm 0.029 $} \\
median2 & $ 0.200 \pm 0.010 $ & $ 0.228 \pm 0.009 $ & $ 0.213 \pm 0.014 $ & $ 0.228 \pm 0.010 $ & $ 0.228 \pm 0.010 $ & {\boldmath$ 0.239 \pm 0.016 $} \\
mestranol\_similarity & $ 0.322 \pm 0.018 $ & $ 0.362 \pm 0.051 $ & $ 0.372 \pm 0.033 $ & $ 0.410 \pm 0.036 $ & $ 0.377 \pm 0.022 $ & {\boldmath$ 0.439 \pm 0.034 $} \\
osimertinib\_mpo & $ 0.741 \pm 0.024 $ & $ 0.781 \pm 0.022 $ & $ 0.771 \pm 0.021 $ & $ 0.802 \pm 0.022 $ & $ 0.781 \pm 0.026 $ & {\boldmath$ 0.830 \pm 0.015 $} \\
perindopril\_mpo & $ 0.444 \pm 0.031 $ & $ 0.501 \pm 0.007 $ & $ 0.487 \pm 0.015 $ & $ 0.488 \pm 0.020 $ & $ 0.488 \pm 0.004 $ & {\boldmath$ 0.535 \pm 0.017 $} \\
qed & $ 0.916 \pm 0.012 $ & {\boldmath$ 0.945 \pm 0.002 $} & $ 0.917 \pm 0.011 $ & $ 0.935 \pm 0.008 $ & $ 0.939 \pm 0.007 $ & $ 0.729 \pm 0.020 $ \\
ranolazine\_mpo & $ 0.595 \pm 0.044 $ & $ 0.767 \pm 0.010 $ & $ 0.628 \pm 0.040 $ & $ 0.759 \pm 0.022 $ & $ 0.749 \pm 0.018 $ & {\boldmath$ 0.781 \pm 0.012 $} \\
scaffold\_hop & $ 0.471 \pm 0.008 $ & $ 0.476 \pm 0.009 $ & $ 0.468 \pm 0.011 $ & $ 0.482 \pm 0.011 $ & $ 0.478 \pm 0.011 $ & {\boldmath$ 0.512 \pm 0.011 $} \\
sitagliptin\_mpo & $ 0.065 \pm 0.015 $ & $ 0.158 \pm 0.039 $ & $ 0.082 \pm 0.038 $ & {\boldmath$ 0.255 \pm 0.042 $} & $ 0.213 \pm 0.055 $ & $ 0.147 \pm 0.037 $ \\
thiothixene\_rediscovery & $ 0.327 \pm 0.032 $ & $ 0.359 \pm 0.009 $ & $ 0.286 \pm 0.034 $ & $ 0.331 \pm 0.012 $ & $ 0.382 \pm 0.009 $ & {\boldmath$ 0.503 \pm 0.030 $} \\
troglitazone\_rediscovery & $ 0.264 \pm 0.007 $ & $ 0.336 \pm 0.010 $ & $ 0.284 \pm 0.012 $ & $ 0.303 \pm 0.012 $ & $ 0.437 \pm 0.108 $ & {\boldmath$ 0.578 \pm 0.107 $} \\
valsartan\_smarts & $ 0.000 \pm 0.000 $ & $ 0.000 \pm 0.000 $ & $ 0.000 \pm 0.000 $ & $ 0.000 \pm 0.000 $ & $ 0.000 \pm 0.000 $ & {\boldmath$ 0.891 \pm 0.026 $} \\
zaleplon\_mpo & $ 0.131 \pm 0.025 $ & $ 0.190 \pm 0.021 $ & $ 0.150 \pm 0.047 $ & {\boldmath$ 0.234 \pm 0.018 $} & $ 0.220 \pm 0.034 $ & $ 0.212 \pm 0.037 $ \\
\midrule
Mean (23 oracles) & $ 0.356 $ & $ 0.443 $ & $ 0.396 $ & $ 0.454 $ & $ 0.464 $ & $ 0.596 $ \\
Oracles won (best of 23) & 0 & 1 & 0 & 2 & 0 & 20 \\
\bottomrule
\end{tabular}
\end{table*}

